Interior-Point Methods Strike Back: Solving the Wasserstein Barycenter Problem

Computing the Wasserstein barycenter of a set of probability measures under the optimal transport metric can quickly become prohibitive for traditional second-order algorithms, such as interior-point methods, as the support size of the measures increases. In this paper, we overcome the difficulty by developing a new adapted interior-point method that fully exploits the problem's special matrix structure to reduce the iteration complexity and speed up the Newton procedure. Different from regularization approaches, our method achieves a well-balanced tradeoff between accuracy and speed. A numerical comparison on various distributions with existing algorithms exhibits the computational advantages of our approach. Moreover, we demonstrate the practicality of our algorithm on image benchmark problems including MNIST and Fashion-MNIST.

==> Newly modified NIPS paper (Final Version Change)/prcipm.tex <==
Predictor-corrector interior point method (PCIPM) \cite{pdipm},  one of the most popular practical interior point methods, on solving (\ref{Regularized Standard LP}).
Set
\begin{equation}\label{vector function}
  F(x,\lambda,s)=\begin{bmatrix} A^{\top}\lambda+s-c\\ Ax-b \\ XS\boldsymbol{1}\end{bmatrix},\text{ and its Jacobian }
  J_F(x,\lambda,s) = \begin{bmatrix} 0&A^{\top}&I\\ A & 0 & 0 \\ S&0&X\end{bmatrix}
\end{equation}
According to Karush–Kuhn–Tucker condition, $x$ is the optimal solution of a linear programming if and only if $F(x,\lambda,s)=\mathbf{0}$. Thus PCIPM is designed to solve this equation, based on the Newton Method and path following strategy.
The general framework of PCIPM is as follows.
\begin{algorithm}[htbp]
	\caption{Predictor-corrector Interior Point Method(PCIPM) }
	\label{Mehrotra's Predictor-corrector Interior Point Method}
    \begin{algorithmic}
    \STATE \textbf{Given} $ (\boldsymbol{x}^0, \boldsymbol{p}^0, \boldsymbol{s}^0)$ with $(\boldsymbol{x}^0, \boldsymbol{s}^0 ) > 0$
    \STATE \textbf{while} a termination criterion is not met, \textbf{do}
    \STATE \quad \textbf{Predictor step}
    \STATE \qquad Solve \begin{equation*}
    J_F(\boldsymbol{x}^k,\boldsymbol{\lambda}^k,\boldsymbol{s}^k)(\Delta \boldsymbol{x}^{\text{aff}},\Delta \boldsymbol{\lambda}^{\text{aff}}, \Delta \boldsymbol{s}^{\text{aff}})^{\top}=-F(\boldsymbol{x}^k,\boldsymbol{\lambda}^k,\boldsymbol{s}^k) \end{equation*}
    \qquad for corrector direction
    $(\Delta\boldsymbol{x}^{\text{aff}},\Delta\boldsymbol{\lambda}^{\text{aff}},\Delta \boldsymbol{s}^{\text{aff}})$;
    \STATE \qquad Calculate \textit{step length} $\mathbf{\alpha}_{\text{aff}}=(\alpha_{\text{aff}}^{\text{pri}}, \alpha_{\text{aff}}^{\text{dual}})$
    such that $(x,s)+(\alpha_{\text{aff}}^{\text{pri}}\Delta x^{\text{aff}},\alpha_{\text{aff}}^{\text{dual}}\Delta s^{\text{aff}}) > 0$;
    \STATE \qquad Calculate \textit{duality measure} $\mu_{\text{aff}} = (x+\alpha_{\text{aff}}^{\text{pri}}\Delta x^{\text{aff}})^{\top}(\lambda + \alpha_{\text{aff}}^{\text{dual}}\Delta s^{\text{aff}})/n$;
    \STATE \qquad Set \textit{centering parameter} $\sigma$;
    \STATE \quad \textbf{Corrector step}
    \STATE \qquad Solve
    \begin{equation*}
      J_F(\boldsymbol{x}^k,\boldsymbol{\lambda}^k,\boldsymbol{s}^k)(\Delta \boldsymbol{x},\Delta \boldsymbol{\lambda}, \Delta \boldsymbol{s})^{\top}=-F(\boldsymbol{x}^k,\boldsymbol{\lambda}^k,\boldsymbol{s}^k) - [0,0,\boldsymbol{1}^{\top}\Delta X^{\text{aff}}\Delta S^{\text{aff}} - \sigma\mu \boldsymbol{1}^{\top}]^{\top}
    \end{equation*}
    \qquad for the \textit{complete Mherotra direction} $(\Delta \boldsymbol{x},\Delta \boldsymbol{\lambda}, \Delta \boldsymbol{s})$;
    \STATE \qquad Calculate \textit{complete step length} $\alpha_k^{\text{pri}}$, $\alpha_k^{\text{dual}}$, $x^{k+1} := x^k+\alpha_k^{\text{pri}}\Delta x$
    \STATE \qquad and $ (\lambda^{k+1},s^{k+1}):=(\lambda^{k},s^{k}) + \alpha_k^{\text{dual}}(\Delta \lambda,\Delta s)$ such as $(x^{k+1},s^{k+1})>0$;
    \STATE \textbf{end(while)}.
    \end{algorithmic}
\end{algorithm}

In PCIPM algorithm \ref{Mehrotra's Predictor-corrector Interior Point Method}, $X$ denotes  $\text{diag}(x_1,x_2,\ldots,x_n)$, $S$ denotes $\text{diag}(s_1,s_2,\ldots,x_n)$ and $\boldsymbol{1}$ denotes  $(1,1,\ldots,1)^{\top}$. For details of the choice of $\mu$ and other parameter in PCIPM see \cite{pdipm}.
The main cost of PCIPM is in solving the linear system of $J_F(\boldsymbol{x}^k,\boldsymbol{\lambda}^k,\boldsymbol{s}^k)$. After reformulating the rows of $J_F(\boldsymbol{x}^k,\boldsymbol{\lambda}^k,\boldsymbol{s}^k)$ , it is cheap to calculate $\Delta s$ and $\Delta x$  while $\Delta \lambda$ requires solving a linear system of the symmetric positive definite matrix $AS^{-1}XA^{\top}$, which is expensive. For most interior point methods, the main cost is in solving this linear system as well, see \cite{PrimalDualIPM}.













%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%aforementioned \textit{Single Low-rank Regularization Method} (SLRM) and \textit{Double Low-rank Regularization Method} (DLRM).
\begin{algorithm}[htbp]
	\caption{PIPM Based Alternating Minimization Algorithm for solving (\ref{non-fix})}
    \label{Alternating Minimizationl Algorithm}
    \begin{algorithmic}
    \STATE \textbf{Input:} Given an initial $X^0$ arbitrarily and set $s=0$
    \STATE \textbf{Pre-solving:} Use the alternating minimization algorithm until $X$ changes little enough between iterations;
    \STATE \textbf{while} a termination criterion of problem (\ref{non-fix}) is not met, \textbf{do}
    \STATE \quad s = 0, choose $(\mathbf{w}^s,\{\pi^{(t),s}\})$ and $\mu^s$ in a certain iteration of the last IPM as a starting point;
    \STATE \quad  \textbf{while} the penalty $\mu^s$ is not sufficiently close to $0$, \textbf{do}
    \STATE \qquad \textbf{while} $(\mathbf{w}^s,\{\pi^{(t),s}\})$ is not sufficiently close to the optimal for (\ref{barrier function}), \textbf{do}
    \STATE \qquad \quad Calculate the Newton direction $p^s$ at $(\mathbf{w}^s,\{\pi^{(t),s}\})$ by \eqref{Newton direction};
    \STATE \qquad\quad $(\mathbf{w}^{s+1},\{\pi^{(t),s+1}\}) = (\mathbf{w}^s,\{\pi^{(t),s}\}) + \alpha^sp^s$, where $\alpha^s$ ensures the interior point; $s = s+1$;
    \STATE \qquad \textbf{end while}
    \STATE \qquad Calculate $X^s$ by (\ref{optimalX}) and choose penalty $\mu^{s+1} < \mu^s$;
    \STATE \quad \textbf{end while}
    \STATE \textbf{end while}
    \STATE \textbf{Output: } $\mathbf{w}^s,X^s,\{\Pi^{(t),s}\}$
    \end{algorithmic}
\end{algorithm}

The pre-solving reduces the change of $X$ after implementing (\ref{optimalX}), which ensures that the first several step lengths $\alpha^s$ in PIPM is sufficiently large.
In PIPM based alternating minimization algorithm, (\ref{optimalX}) can be computed in every iteration instead of every whole linear programming, which largely save the cost of time. We remain $X$ and restart $(\mathbf{w}^s,\{\pi^{(t),s}\})$  from a certain iteration of the last PIPM for several times trying to jump out of the local minimizer or saddle point. Numerical studies show that the PIPM based alternating minimization algorithm outperforms the previous free support case algorithms in both speed and accuracy.












\textbf{Primal-dual interior point method for pre-specified support cases.}
We briefly introduce the framework of primal-dual interior point methods on solving \eqref{Regularized Standard LP}. 
Set
\begin{equation}\label{vector function}
  F(\boldsymbol{x},\boldsymbol{\lambda},\boldsymbol{s})=\begin{bmatrix} \bar{A}^{\top}\boldsymbol{\lambda}+\boldsymbol{s}-\boldsymbol{c}\\ \bar{A}\boldsymbol{x}-\boldsymbol{b} \\ XS\boldsymbol{1}\end{bmatrix},\text{ and its Jacobian }
  J_F(\boldsymbol{x},\boldsymbol{\lambda},\boldsymbol{s}) = \begin{bmatrix} 0&\bar{A}^{\top}&I\\ \bar{A} & 0 & 0 \\ S&0&X\end{bmatrix},
\end{equation}
where $X$ denotes  $\text{diag}(x_1,x_2,\ldots,x_n)$, $S$ denotes $\text{diag}(s_1,s_2,\ldots,x_n)$ and $\boldsymbol{1}$ denotes $(1,1,\ldots,1)^{\top}$.
According to Karush–Kuhn–Tucker condition, $x$ is the optimal solution of a linear programming if and only if $F(\boldsymbol{x},\boldsymbol{\lambda},\boldsymbol{s})=\mathbf{0}$. Thus interior point methods are designed to solve this equation, based on the Newton method and path following strategy. In the $k^{th}$ iteration, $(\Delta \boldsymbol{x}_{k},\Delta \boldsymbol{\lambda}_{k}, \Delta \boldsymbol{s}_k)$ is computed by
\begin{equation}\label{IPM iterate}
    J_F(\boldsymbol{x}_k,\boldsymbol{\lambda}_k,\boldsymbol{s}_k)(\Delta \boldsymbol{x}_k,\Delta \boldsymbol{\lambda}_k, \Delta \boldsymbol{s}_k)^{\top}
    =-F(\boldsymbol{x}_k,\boldsymbol{\lambda}_k,\boldsymbol{s}_k) +[0,0,\sigma\mu\boldsymbol{1}^{\top}]^{\top},
\end{equation}
where a \textit{duality measure} $\mu$ is $\boldsymbol{x}^{\top}\boldsymbol{s}/n$, and a \textit{centering parameter} $\sigma$ is decreased in every iteration, defined in \cite{book}.
In solving \eqref{Standard LP}, a feasible initial point $(\boldsymbol{x}^0, \boldsymbol{\lambda}^0, \boldsymbol{s}^0)$ can be easily found by 
\begin{equation}\label{initial point}
    \text{\color{SkyBlue}initial feasible point... to be finished}.
\end{equation}
So \eqref{IPM iterate} can be reformulated by 
\begin{equation}\label{ADAsystem}
    \bar{A}{D_k}^2\bar{A}\Delta \boldsymbol{\lambda}_k = \bar{A}(\boldsymbol{x}_k-\sigma\mu{S_{k}}^{-1}\boldsymbol{1}),
\end{equation}
$\Delta \boldsymbol{s}_k = - \bar{A}^{\top}\Delta \boldsymbol{\lambda}_k$, $\Delta \boldsymbol{x}_k = -\boldsymbol{x}_k + \sigma\mu S^{-1}\boldsymbol{1} - {S_k}^{-1}X_k\Delta \boldsymbol{s}_k$, and $D_k = {S_k}^{-1}X_k$. Note that the main cost of most variants of primal-dual interior point methods lies in solving the linear system \eqref{ADAsystem}. 
%In the following subsections, we will provide two highly efficient methods to solve this linear system.
In practice, we develop a primal-dual Matrix-based Interior Point Method(pd-MIPM), which follows the framework of predictor-corrector interior point method in \cite{pdipm} but largely reduces the main cost of solving \eqref{ADAsystem} by the two highly efficient methods in section \ref{Efficient Methods for Solving the Normal Equations}.


\textbf{Primal interior point method for unknown support cases.}\label{free support problem}
For the cases that the support points are not pre-specified, we need to solve problem \eqref{non-fix}. When $X$ is fixed, the problem is a linear programming.
%, which can be efficiently solved by algorithm \ref{Mehrotra's Predictor-corrector Interior Point Method}. 
When $(\mathbf{w},\{\Pi^t\})$ are fixed, the problem is a quadratic optimization problem with respect to $X$, and the optimal $X^*$ can be written in closed form
\begin{equation}\label{optimalX}
  \textstyle\mathbf{x}_i^* = \big(\sum_{t=1}^{N}\sum_{j=1}^{m_t}\pi_{ij}^{(t)}\big)^{-1}{\sum_{t=1}^{N}\sum_{j=1}^{m_t}\pi_{ij}^{(t)}\mathbf{q}_{j}^{(t)}},\quad i=1,2\ldots,m.
\end{equation}
In fact, \eqref{non-fix} is a non-convex problem, in which contains saddle points and local minimizers, so it is difficult to find the global optimizer of problem \eqref{non-fix}. Examples are available in the supplement.
The alternating minimization strategy used in \cite{Cuturi-2014-OTbarycenter,sGS-ADMM,scaling up discrete,B-ADMM}
%\textit{pd-MIPM based alternating minimization} (PCIPMAM) 
alternates the proceeds of optimizing $X$ by \eqref{optimalX} and optimizing $(\mathbf{w}^{s+1},\{\Pi^{(t),s+1}\})$ in problem (\ref{fix}).
But it cannot avoid either local minimizers or saddle points, and every iteration may require solving a complete linear programming \eqref{fix}, which is expensive.
The pd-MIPM Alternating Minimization (pd-MIPMAM) adopts this strategy. After optimizing the support points, in order to take use of the last pd-MIPM, some warm-start strategies \cite{warm start, imple warm} can be implemented. However, these warm-start strategies can only save the computational time slightly, as Table 4 in \cite{imple warm}, and they require storing $\boldsymbol{x}, ~\boldsymbol{s}$ in the back-tracing iterations, which is not memory efficient.

To solve the drawbacks, we propose a new algorithm, namely primal Matrix-based Interior Point Method (p-MIPM). The p-MIPM follow the framework of primal interior point method stated in \cite{PrimalIPM}. It combines the proceed of following the central path with optimizing the support points,i.e., it contains three parts, optimizing the logarithmic barrier function
\begin{equation}\label{barrier function}
\textstyle  \text{minimize}\quad \boldsymbol{c}^{\top}\boldsymbol{x}-\mu\sum_{i=1}^{n}\ln {x}_i,\quad \text{subject to}\quad \bar{A}\boldsymbol{x} = \boldsymbol{b},
\end{equation}
 reducing the penalty $\mu$, and calculating the support \eqref{optimalX}. Applying Newton method to solve (\ref{barrier function}), Newton direction $\boldsymbol{p}_k$ at the $k^{th}$ iteration is calculate by
\begin{equation}\label{Newton direction}
\textstyle  \boldsymbol{p}_k = \boldsymbol{x}_k+X_k^2\big(\bar{A}^{\top}{(\bar{A}X_k^2\bar{A}^{\top})}^{-1}(\bar{A}X_k^2c-\mu \bar{A}X_k\boldsymbol{1})\big)/\mu_k.
\end{equation}
The main cost of p-MIPM lies in solving a linear system of $AX^2\bar{A}$, which can be fast solved by the two methods in the following section as well.
In practice, we use a presolve phase that pd-MIPMAM are used until the support changes little enough between iterations, which ensures that the first several step lengths in p-MIPM is sufficiently large.
In p-MIPM. (\ref{optimalX}) can be computed in every iteration instead of every whole linear programming, which largely saves the cost of time.
After implementing one p-MIPM, if the termination criterion is not met, we can implement another p-MIPM trying to jump out of the local minimizers. In practice, we apply a warm-start strategy, choosing the new support points and the $(\mathbf{w}^s,\{\pi^{(t),s}\}), \mu^s$ in a certain iteration of the last p-MIPM as the starting point of the next p-MIPM. 
Compared with primal-dual IPMs' warm-start strategies \cite{warm start, imple warm}, this strategy saves the searching time, and only requires slightly more memory.
Numerical studies show that this algorithm, namely the p-MIPM Based Alternating Minimization Algorithm(p-MIPMAM), outperforms the previous free support case algorithms in both speed and accuracy.

==> prcipm.tex <==
Predictor-corrector interior point method (PCIPM) \cite{pdipm},  one of the most popular practical interior point methods, on solving (\ref{Regularized Standard LP}).
Set
\begin{equation}\label{vector function}
  F(x,\lambda,s)=\begin{bmatrix} A^{\top}\lambda+s-c\\ Ax-b \\ XS\boldsymbol{1}\end{bmatrix},\text{ and its Jacobian }
  J_F(x,\lambda,s) = \begin{bmatrix} 0&A^{\top}&I\\ A & 0 & 0 \\ S&0&X\end{bmatrix}
\end{equation}
According to Karush–Kuhn–Tucker condition, $x$ is the optimal solution of a linear programming if and only if $F(x,\lambda,s)=\mathbf{0}$. Thus PCIPM is designed to solve this equation, based on the Newton Method and path following strategy.
The general framework of PCIPM is as follows.
\begin{algorithm}[htbp]
	\caption{Predictor-corrector Interior Point Method(PCIPM) }
	\label{Mehrotra's Predictor-corrector Interior Point Method}
    \begin{algorithmic}
    \STATE \textbf{Given} $ (\boldsymbol{x}^0, \boldsymbol{p}^0, \boldsymbol{s}^0)$ with $(\boldsymbol{x}^0, \boldsymbol{s}^0 ) > 0$
    \STATE \textbf{while} a termination criterion is not met, \textbf{do}
    \STATE \quad \textbf{Predictor step}
    \STATE \qquad Solve \begin{equation*}
    J_F(\boldsymbol{x}^k,\boldsymbol{\lambda}^k,\boldsymbol{s}^k)(\Delta \boldsymbol{x}^{\text{aff}},\Delta \boldsymbol{\lambda}^{\text{aff}}, \Delta \boldsymbol{s}^{\text{aff}})^{\top}=-F(\boldsymbol{x}^k,\boldsymbol{\lambda}^k,\boldsymbol{s}^k) \end{equation*}
    \qquad for corrector direction
    $(\Delta\boldsymbol{x}^{\text{aff}},\Delta\boldsymbol{\lambda}^{\text{aff}},\Delta \boldsymbol{s}^{\text{aff}})$;
    \STATE \qquad Calculate \textit{step length} $\mathbf{\alpha}_{\text{aff}}=(\alpha_{\text{aff}}^{\text{pri}}, \alpha_{\text{aff}}^{\text{dual}})$
    such that $(x,s)+(\alpha_{\text{aff}}^{\text{pri}}\Delta x^{\text{aff}},\alpha_{\text{aff}}^{\text{dual}}\Delta s^{\text{aff}}) > 0$;
    \STATE \qquad Calculate \textit{duality measure} $\mu_{\text{aff}} = (x+\alpha_{\text{aff}}^{\text{pri}}\Delta x^{\text{aff}})^{\top}(\lambda + \alpha_{\text{aff}}^{\text{dual}}\Delta s^{\text{aff}})/n$;
    \STATE \qquad Set \textit{centering parameter} $\sigma$;
    \STATE \quad \textbf{Corrector step}
    \STATE \qquad Solve
    \begin{equation*}
      J_F(\boldsymbol{x}^k,\boldsymbol{\lambda}^k,\boldsymbol{s}^k)(\Delta \boldsymbol{x},\Delta \boldsymbol{\lambda}, \Delta \boldsymbol{s})^{\top}=-F(\boldsymbol{x}^k,\boldsymbol{\lambda}^k,\boldsymbol{s}^k) - [0,0,\boldsymbol{1}^{\top}\Delta X^{\text{aff}}\Delta S^{\text{aff}} - \sigma\mu \boldsymbol{1}^{\top}]^{\top}
    \end{equation*}
    \qquad for the \textit{complete Mherotra direction} $(\Delta \boldsymbol{x},\Delta \boldsymbol{\lambda}, \Delta \boldsymbol{s})$;
    \STATE \qquad Calculate \textit{complete step length} $\alpha_k^{\text{pri}}$, $\alpha_k^{\text{dual}}$, $x^{k+1} := x^k+\alpha_k^{\text{pri}}\Delta x$
    \STATE \qquad and $ (\lambda^{k+1},s^{k+1}):=(\lambda^{k},s^{k}) + \alpha_k^{\text{dual}}(\Delta \lambda,\Delta s)$ such as $(x^{k+1},s^{k+1})>0$;
    \STATE \textbf{end(while)}.
    \end{algorithmic}
\end{algorithm}

In PCIPM algorithm \ref{Mehrotra's Predictor-corrector Interior Point Method}, $X$ denotes  $\text{diag}(x_1,x_2,\ldots,x_n)$, $S$ denotes $\text{diag}(s_1,s_2,\ldots,x_n)$ and $\boldsymbol{1}$ denotes  $(1,1,\ldots,1)^{\top}$. For details of the choice of $\mu$ and other parameter in PCIPM see \cite{pdipm}.
The main cost of PCIPM is in solving the linear system of $J_F(\boldsymbol{x}^k,\boldsymbol{\lambda}^k,\boldsymbol{s}^k)$. After reformulating the rows of $J_F(\boldsymbol{x}^k,\boldsymbol{\lambda}^k,\boldsymbol{s}^k)$ , it is cheap to calculate $\Delta s$ and $\Delta x$  while $\Delta \lambda$ requires solving a linear system of the symmetric positive definite matrix $AS^{-1}XA^{\top}$, which is expensive. For most interior point methods, the main cost is in solving this linear system as well, see \cite{PrimalDualIPM}.













%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%aforementioned \textit{Single Low-rank Regularization Method} (SLRM) and \textit{Double Low-rank Regularization Method} (DLRM).
\begin{algorithm}[htbp]
	\caption{PIPM Based Alternating Minimization Algorithm for solving (\ref{non-fix})}
    \label{Alternating Minimizationl Algorithm}
    \begin{algorithmic}
    \STATE \textbf{Input:} Given an initial $X^0$ arbitrarily and set $s=0$
    \STATE \textbf{Pre-solving:} Use the alternating minimization algorithm until $X$ changes little enough between iterations;
    \STATE \textbf{while} a termination criterion of problem (\ref{non-fix}) is not met, \textbf{do}
    \STATE \quad s = 0, choose $(\mathbf{w}^s,\{\pi^{(t),s}\})$ and $\mu^s$ in a certain iteration of the last IPM as a starting point;
    \STATE \quad  \textbf{while} the penalty $\mu^s$ is not sufficiently close to $0$, \textbf{do}
    \STATE \qquad \textbf{while} $(\mathbf{w}^s,\{\pi^{(t),s}\})$ is not sufficiently close to the optimal for (\ref{barrier function}), \textbf{do}
    \STATE \qquad \quad Calculate the Newton direction $p^s$ at $(\mathbf{w}^s,\{\pi^{(t),s}\})$ by \eqref{Newton direction};
    \STATE \qquad\quad $(\mathbf{w}^{s+1},\{\pi^{(t),s+1}\}) = (\mathbf{w}^s,\{\pi^{(t),s}\}) + \alpha^sp^s$, where $\alpha^s$ ensures the interior point; $s = s+1$;
    \STATE \qquad \textbf{end while}
    \STATE \qquad Calculate $X^s$ by (\ref{optimalX}) and choose penalty $\mu^{s+1} < \mu^s$;
    \STATE \quad \textbf{end while}
    \STATE \textbf{end while}
    \STATE \textbf{Output: } $\mathbf{w}^s,X^s,\{\Pi^{(t),s}\}$
    \end{algorithmic}
\end{algorithm}

The pre-solving reduces the change of $X$ after implementing (\ref{optimalX}), which ensures that the first several step lengths $\alpha^s$ in PIPM is sufficiently large.
In PIPM based alternating minimization algorithm, (\ref{optimalX}) can be computed in every iteration instead of every whole linear programming, which largely save the cost of time. We remain $X$ and restart $(\mathbf{w}^s,\{\pi^{(t),s}\})$  from a certain iteration of the last PIPM for several times trying to jump out of the local minimizer or saddle point. Numerical studies show that the PIPM based alternating minimization algorithm outperforms the previous free support case algorithms in both speed and accuracy.












\textbf{Primal-dual interior point method for pre-specified support cases.}
We briefly introduce the framework of primal-dual interior point methods on solving \eqref{Regularized Standard LP}. 
Set
\begin{equation}\label{vector function}
  F(\boldsymbol{x},\boldsymbol{\lambda},\boldsymbol{s})=\begin{bmatrix} \bar{A}^{\top}\boldsymbol{\lambda}+\boldsymbol{s}-\boldsymbol{c}\\ \bar{A}\boldsymbol{x}-\boldsymbol{b} \\ XS\boldsymbol{1}\end{bmatrix},\text{ and its Jacobian }
  J_F(\boldsymbol{x},\boldsymbol{\lambda},\boldsymbol{s}) = \begin{bmatrix} 0&\bar{A}^{\top}&I\\ \bar{A} & 0 & 0 \\ S&0&X\end{bmatrix},
\end{equation}
where $X$ denotes  $\text{diag}(x_1,x_2,\ldots,x_n)$, $S$ denotes $\text{diag}(s_1,s_2,\ldots,x_n)$ and $\boldsymbol{1}$ denotes $(1,1,\ldots,1)^{\top}$.
According to Karush–Kuhn–Tucker condition, $x$ is the optimal solution of a linear programming if and only if $F(\boldsymbol{x},\boldsymbol{\lambda},\boldsymbol{s})=\mathbf{0}$. Thus interior point methods are designed to solve this equation, based on the Newton method and path following strategy. In the $k^{th}$ iteration, $(\Delta \boldsymbol{x}_{k},\Delta \boldsymbol{\lambda}_{k}, \Delta \boldsymbol{s}_k)$ is computed by
\begin{equation}\label{IPM iterate}
    J_F(\boldsymbol{x}_k,\boldsymbol{\lambda}_k,\boldsymbol{s}_k)(\Delta \boldsymbol{x}_k,\Delta \boldsymbol{\lambda}_k, \Delta \boldsymbol{s}_k)^{\top}
    =-F(\boldsymbol{x}_k,\boldsymbol{\lambda}_k,\boldsymbol{s}_k) +[0,0,\sigma\mu\boldsymbol{1}^{\top}]^{\top},
\end{equation}
where a \textit{duality measure} $\mu$ is $\boldsymbol{x}^{\top}\boldsymbol{s}/n$, and a \textit{centering parameter} $\sigma$ is decreased in every iteration, defined in \cite{book}.
In solving \eqref{Standard LP}, a feasible initial point $(\boldsymbol{x}^0, \boldsymbol{\lambda}^0, \boldsymbol{s}^0)$ can be easily found by 
\begin{equation}\label{initial point}
    \text{\color{SkyBlue}initial feasible point... to be finished}.
\end{equation}
So \eqref{IPM iterate} can be reformulated by 
\begin{equation}\label{ADAsystem}
    \bar{A}{D_k}^2\bar{A}\Delta \boldsymbol{\lambda}_k = \bar{A}(\boldsymbol{x}_k-\sigma\mu{S_{k}}^{-1}\boldsymbol{1}),
\end{equation}
$\Delta \boldsymbol{s}_k = - \bar{A}^{\top}\Delta \boldsymbol{\lambda}_k$, $\Delta \boldsymbol{x}_k = -\boldsymbol{x}_k + \sigma\mu S^{-1}\boldsymbol{1} - {S_k}^{-1}X_k\Delta \boldsymbol{s}_k$, and $D_k = {S_k}^{-1}X_k$. Note that the main cost of most variants of primal-dual interior point methods lies in solving the linear system \eqref{ADAsystem}. 
%In the following subsections, we will provide two highly efficient methods to solve this linear system.
In practice, we develop a primal-dual Matrix-based Interior Point Method(pd-MIPM), which follows the framework of predictor-corrector interior point method in \cite{pdipm} but largely reduces the main cost of solving \eqref{ADAsystem} by the two highly efficient methods in section \ref{Efficient Methods for Solving the Normal Equations}.


\textbf{Primal interior point method for unknown support cases.}\label{free support problem}
For the cases that the support points are not pre-specified, we need to solve problem \eqref{non-fix}. When $X$ is fixed, the problem is a linear programming.
%, which can be efficiently solved by algorithm \ref{Mehrotra's Predictor-corrector Interior Point Method}. 
When $(\mathbf{w},\{\Pi^t\})$ are fixed, the problem is a quadratic optimization problem with respect to $X$, and the optimal $X^*$ can be written in closed form
\begin{equation}\label{optimalX}
  \textstyle\mathbf{x}_i^* = \big(\sum_{t=1}^{N}\sum_{j=1}^{m_t}\pi_{ij}^{(t)}\big)^{-1}{\sum_{t=1}^{N}\sum_{j=1}^{m_t}\pi_{ij}^{(t)}\mathbf{q}_{j}^{(t)}},\quad i=1,2\ldots,m.
\end{equation}
In fact, \eqref{non-fix} is a non-convex problem, in which contains saddle points and local minimizers, so it is difficult to find the global optimizer of problem \eqref{non-fix}. Examples are available in the supplement.
The alternating minimization strategy used in \cite{Cuturi-2014-OTbarycenter,sGS-ADMM,scaling up discrete,B-ADMM}
%\textit{pd-MIPM based alternating minimization} (PCIPMAM) 
alternates the proceeds of optimizing $X$ by \eqref{optimalX} and optimizing $(\mathbf{w}^{s+1},\{\Pi^{(t),s+1}\})$ in problem (\ref{fix}).
But it cannot avoid either local minimizers or saddle points, and every iteration may require solving a complete linear programming \eqref{fix}, which is expensive.
The pd-MIPM Alternating Minimization (pd-MIPMAM) adopts this strategy. After optimizing the support points, in order to take use of the last pd-MIPM, some warm-start strategies \cite{warm start, imple warm} can be implemented. However, these warm-start strategies can only save the computational time slightly, as Table 4 in \cite{imple warm}, and they require storing $\boldsymbol{x}, ~\boldsymbol{s}$ in the back-tracing iterations, which is not memory efficient.

To solve the drawbacks, we propose a new algorithm, namely primal Matrix-based Interior Point Method (p-MIPM). The p-MIPM follow the framework of primal interior point method stated in \cite{PrimalIPM}. It combines the proceed of following the central path with optimizing the support points,i.e., it contains three parts, optimizing the logarithmic barrier function
\begin{equation}\label{barrier function}
\textstyle  \text{minimize}\quad \boldsymbol{c}^{\top}\boldsymbol{x}-\mu\sum_{i=1}^{n}\ln {x}_i,\quad \text{subject to}\quad \bar{A}\boldsymbol{x} = \boldsymbol{b},
\end{equation}
 reducing the penalty $\mu$, and calculating the support \eqref{optimalX}. Applying Newton method to solve (\ref{barrier function}), Newton direction $\boldsymbol{p}_k$ at the $k^{th}$ iteration is calculate by
\begin{equation}\label{Newton direction}
\textstyle  \boldsymbol{p}_k = \boldsymbol{x}_k+X_k^2\big(\bar{A}^{\top}{(\bar{A}X_k^2\bar{A}^{\top})}^{-1}(\bar{A}X_k^2c-\mu \bar{A}X_k\boldsymbol{1})\big)/\mu_k.
\end{equation}
The main cost of p-MIPM lies in solving a linear system of $AX^2\bar{A}$, which can be fast solved by the two methods in the following section as well.
In practice, we use a presolve phase that pd-MIPMAM are used until the support changes little enough between iterations, which ensures that the first several step lengths in p-MIPM is sufficiently large.
In p-MIPM. (\ref{optimalX}) can be computed in every iteration instead of every whole linear programming, which largely saves the cost of time.
After implementing one p-MIPM, if the termination criterion is not met, we can implement another p-MIPM trying to jump out of the local minimizers. In practice, we apply a warm-start strategy, choosing the new support points and the $(\mathbf{w}^s,\{\pi^{(t),s}\}), \mu^s$ in a certain iteration of the last p-MIPM as the starting point of the next p-MIPM. 
Compared with primal-dual IPMs' warm-start strategies \cite{warm start, imple warm}, this strategy saves the searching time, and only requires slightly more memory.
Numerical studies show that this algorithm, namely the p-MIPM Based Alternating Minimization Algorithm(p-MIPMAM), outperforms the previous free support case algorithms in both speed and accuracy.
